On the Extent, Correlates, and Consequences of Reporting Bias in Survey Wages

Surveys are an indispensable source of data for applied economic research; however, their reliance on self-reported information can introduce bias, especially if core variables such as personal income are misreported. To assess the extent and impact of this misreporting bias, we compare self-reported wages from the German Socio-Economic Panel (SOEP) with administrative wages from social security records (IEB) for the same individuals. Using a novel and unique data linkage (SOEP-ADIAB), we identify a modest but economically significant reporting bias, with SOEP respondents underreporting their administrative wages by about 7.3%. This misreporting varies systematically with individual, household, and especially job and firm characteristics. In replicating common empirical analyses in which wages serve as either dependent or independent variables, we find that misreporting is consequential for some, but not all estimated relationships. It turns out to be inconsequential for examining the returns to education, but relevant for analyzing the gender wage gap. In addition we find that misreporting bias can significantly affect the results when wage is used as the independent variable. Specifically, estimates of the wage-satisfaction relationship are substantially overestimated when based on survey data, although this bias is mitigated when focusing on interpersonal changes. Our findings underscore that survey-based measures of individual wages can significantly bias commonly estimated empirical relationships. They also demonstrate the enormous research potential of linked administrative-survey data.

==> tables/02_reliability_measure.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{8}{c}}
\toprule
            &\multicolumn{2}{c}{All}                    &\multicolumn{2}{c}{Tercile 1}              &\multicolumn{2}{c}{Tercile 2}              &\multicolumn{2}{c}{Tercile 3}              \\                                     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}          
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
            &\multicolumn{1}{c}{\shortstack{SOEP\\Wage}}&\multicolumn{1}{c}{\shortstack{$\Delta$~SOEP\\Wage}}&\multicolumn{1}{c}{\shortstack{SOEP\\Wage}}&\multicolumn{1}{c}{\shortstack{$\Delta$~SOEP\\Wage}}&\multicolumn{1}{c}{\shortstack{SOEP\\Wage}}&\multicolumn{1}{c}{\shortstack{$\Delta$~SOEP\\Wage}}&\multicolumn{1}{c}{\shortstack{SOEP\\Wage}}&\multicolumn{1}{c}{\shortstack{$\Delta$~SOEP\\Wage}}\\
\midrule
IEB Wage    &       0.911\sym{***}&                     &       1.011\sym{***}&                     &       0.938\sym{***}&                     &       0.897\sym{***}&                     \\
            &     (0.038)         &                     &     (0.307)         &                     &     (0.074)         &                     &     (0.031)         &                     \\
\addlinespace
$\Delta$~IEB Wage&                     &      -0.021\sym{***}         &                     &      -0.031\sym{***}         &                     &      -0.060\sym{***}         &                     &      -0.006         \\
            &                     &     (0.015)         &                     &     (0.028)         &                     &     (0.039)         &                     &     (0.019)         \\
\midrule
N           &         690         &         370         &         230         &         125         &         230         &         117         &         230         &         128         \\
R2          &        0.43         &        0.01         &        0.58         &        0.01         &        0.72         &        0.02         &        0.67         &        0.00         \\
Mean dep. var.&     2178.58         &       86.44         &     2208.15         &       94.31         &     2207.70         &       88.55         &     2119.88         &       76.82         \\
\bottomrule
\end{tabular}
}

